Random Variate Generation with Formal Guarantees

This article introduces a new approach to principled and practical random variate generation with formal guarantees. The key idea is to first specify the desired probability distribution in terms of a finite-precision numerical program that defines its cumulative distribution function (CDF), and then generate exact random variates according to this CDF. We present a universal and fully automated method to synthesize exact random variate generators given any numerical CDF implemented in any binary number format, such as floating-point, fixed-point, and posits. The method is guaranteed to operate with the same precision used to specify the CDF, does not overflow, avoids expensive arbitrary-precision arithmetic, and exposes a consistent API. The method rests on a novel space-time optimal implementation for the class of generators that attain the information-theoretically optimal Knuth and Yao entropy rate, consuming the least possible number of input random bits per output variate. We develop a random variate generation library using our method in C and evaluate it on a diverse set of ``continuous'' and ``discrete'' distributions, showing competitive runtime with the state-of-the-art GNU Scientific Library while delivering higher accuracy, entropy efficiency, and automation.

==> Makefile <==
DOC  := paper.tex
TARGET := paper.pdf
PRODUCTS := $(TARGET) submission.pdf appendix.pdf abstract pldi25main-p38-p.pdf

SOURCES := $(shell \
	git -c grep.lineNumber=false grep -P '^\\input\{' -- ':(exclude)*.cls' \
	| sed 's/.*\input{//g' | sed 's/\}//g' \
	| xargs -I% echo %.tex \
	| sort)

FIGURES := $(shell git grep -P '\\includegraphics.*\{.*\}' | grep -o -P 'assets/.*\.(pdf|png)')

EXTRAS := paper.bbl paper.bib acmart.cls ACM-Reference-Format.bst Makefile

$(TARGET): $(SOURCES) $(FIGURES)
	latexmk -pdf $(DOC)

bookmarks.txt: $(TARGET)
	pdftk paper.pdf dump_data_utf8 \
		| grep -P '^Bookmark' \
		| awk 'found && NR > start+2 { exit } /^BookmarkTitle: References/ && !found { start=NR; found=1 } { print }' \
		> bookmarks.txt

submission: $(TARGET) bookmarks.txt
	pdftk $(TARGET) cat 1-25 output submission.pdf
	pdftk $(TARGET) cat 26-end output appendix.pdf
	pdftk submission.pdf update_info bookmarks.txt output main.pdf
	rm submission.pdf
	cp $(TARGET) pldi25main-p38-p.pdf

clean:
	latexmk -C *.tex
	rm -f *.{aux,dvi,log,bbl,blg,brf,fls,toc,thm,out,fdb_latexmk}
	rm -f $(PRODUCTS)

abstract: $(DOC)
	@sed -n \
		'/\\begin{abstract}/,/\\end{abstract}/p' "$(DOC)" \
		| sed '/\\begin{abstract}/d;/\\end{abstract}/d;/^%/d' \
		| sed -z 's/\n\n/PLACEHOLDER/g; s/\n/ /g; s/PLACEHOLDER/\n\n/g; s/ $$//' \
		| sed '$$a\' \
		| sed 's/\\citeauthor{knuth1976}/Knuth and Yao/g'\
		| tee abstract

arxiv.zip: ${TARGET} ${SOURCES} ${FIGURES}
	rm -rf arxiv.zip
	zip arxiv.zip ${DOC} ${SOURCES} ${FIGURES} ${EXTRAS}

.PHONY: clean submission

